Enhancing Pre-trained ASR System Fine-tuning for Dysarthric Speech Recognition using Adversarial Data Augmentation

Automatic recognition of dysarthric speech remains a highly challenging task to date. Neuro-motor conditions and co-occurring physical disabilities create difficulty in large-scale data collection for ASR system development. Adapting SSL pre-trained ASR models to limited dysarthric speech via data-intensive parameter fine-tuning leads to poor generalization. To this end, this paper presents an extensive comparative study of various data augmentation approaches to improve the robustness of pre-trained ASR model fine-tuning to dysarthric speech. These include: a) conventional speaker-independent perturbation of impaired speech; b) speaker-dependent speed perturbation, or GAN-based adversarial perturbation of normal, control speech based on their time alignment against parallel dysarthric speech; c) novel Spectral basis GAN-based adversarial data augmentation operating on non-parallel data. Experiments conducted on the UASpeech corpus suggest GAN-based data augmentation consistently outperforms fine-tuned Wav2vec2.0 and HuBERT models using no data augmentation and speed perturbation across different data expansion operating points by statistically significant word error rate (WER) reductions up to 2.01% and 0.96% absolute (9.03% and 4.63% relative) respectively on the UASpeech test set of 16 dysarthric speakers. After cross-system outputs rescoring, the best system produced the lowest published WER of 16.53% (46.47% on very low intelligibility) on UASpeech.

==> Table/tab2.tex <==
\begin{table}[!t]
    \caption{``Sys. W$\rightarrow$X$\rightarrow$Y$\rightarrow$Z'' in the second column denotes the N-best (N=100) outputs of TDNN W are further rescored by Conformer X, Wav2vec2.0 Y and HuBERT Z via two-pass decoding \cite{cui2022two} (Sys. 1-3). Sys. 4 denotes a further combination of Sys. 1-3 from this table. ``$\dag$'' denotes a statis. sig. WER difference is obtained from Sys. 1-4 against Sys. 23 from Table \ref{tab:WAV2VEC}. Other naming conventions follow the one adopted in Table \ref{tab:WAV2VEC}.}
    \label{tab:rescoring}
    \centering
    \vspace{-0.3cm}
    \scalebox{0.89}{\begin{tabular}{c|c|c|cccc|c}
    \hline\hline
    \multirow{2}{*}{Sys.} & \multirow{2}{*}{DA} & \multirow{2}{*}{Model} & \multicolumn{5}{c}{Word Error Rate \%} \\
    \cline{4-8}
     & & & VL & L & M & H & Avg. \\
    \hline\hline
    1 & S & Sys. 5$\rightarrow$12$\rightarrow$17$\rightarrow$22, Table \ref{tab:WAV2VEC} & 48.84$^\dag$ & 16.73$^\dag$ & 7.29$^\dag$ & 3.08 & 17.12$^\dag$ \\
    2 & SG & Sys. 6$\rightarrow$13$\rightarrow$18$\rightarrow$23, Table \ref{tab:WAV2VEC} & 46.90$^\dag$ & 17.34$^\dag$ & 6.71$^\dag$ & 2.91 & 16.69$^\dag$ \\
    3 & SBG & Sys. 7$\rightarrow$14$\rightarrow$19$\rightarrow$24, Table \ref{tab:WAV2VEC} & 47.99$^\dag$ & 17.08$^\dag$ & 7.80$^\dag$ & 2.85 & 17.04$^\dag$ \\
    \hline\hline
    4 & All & Sys. 1$\rightarrow$2$\rightarrow$3 & 46.47$^\dag$ & 16.76$^\dag$ & 7.18$^\dag$ & 2.89 & 16.53$^\dag$ \\
    \hline\hline
    \end{tabular}}
    \vspace{-7.5mm}
\end{table}

